LL-GABR: Energy Efficient Live Video Streaming Using Reinforcement Learning

Over the recent years, research and development in adaptive bitrate (ABR) algorithms for live video streaming have been successful in improving users' quality of experience (QoE) by reducing latency to near real-time levels while delivering higher bitrate videos with minimal rebuffering time. However, the QoE models used by these ABR algorithms do not take into account that a large portion of live video streaming clients use mobile devices where a higher bitrate does not necessarily translate into higher perceived quality. Ignoring perceived quality results in playing videos at higher bitrates without a significant increase in perceptual video quality and becomes a burden for battery-constrained mobile devices due to higher energy consumption. In this paper, we propose LL-GABR, a deep reinforcement learning approach that models the QoE using perceived video quality instead of bitrate and uses energy consumption along with other metrics like latency, rebuffering events, and smoothness. LL-GABR makes no assumptions about the underlying video, environment, or network settings and can operate flexibly on different video titles, each having a different bitrate encoding ladder without additional re-training, unlike existing learning-based ABRs. Trace-driven experimental results show that LL-GABR outperforms the state-of-the-art approaches by up to 44% in terms of perceptual QoE and a 73% increase in energy efficiency as a result of reducing net energy consumption by 11%.

==> mega_table_1.tex <==
\begin{table*}[ht]
\centering
\small
% \rowcolors{3}{gray!25}{white}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\begin{tabular}{c|c|ccccccccc}
% \begin{tabular}{|c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|}
     
% \begin{tabular}{*11c}
\hline

% Heading row #1
% \rowcolor{white}
& \multirow{2}{*}{\textbf{ABR}} & 
\multirow{1}{*}{\textbf{Quality}} & 
\multirow{1}{*}{\textbf{Quality}} & 
\multirow{1}{*}{\textbf{Data}} & 
\multirow{1}{*}{\textbf{Latency}} & 
\multirow{2}{*}{\textbf{Speed}} & 
\multirow{1}{*}{\textbf{Freezing}} & 
\multirow{1}{*}{\textbf{Energy}} & 
\multirow{2}{*}{\textbf{QoE}} & 
\multirow{1}{*}{\textbf{Energy}} \\

% Heading row #2
% \rowcolor{white}
&  & \textbf{level} (0-5) & \textbf{Smooth} & \textbf{dl} \textit{(in Mb)} & \textit{(sec)} & & \textit{(sec)}  & \textit{(kj)} & & \textbf{Efficiency} \\
\hline
\multirow{5}{*}{\rotatebox{90}{\textbf{Animation}}}
    & {\ProjectName} & 
         4.5{\scriptsize$\pm$0.18} & \cellcolor{green!30}{10.6\scriptsize{$\pm$12.2} $\downarrow$}  & \cellcolor{green!30}{75.6\scriptsize{$\pm$19.7} $\downarrow$} & 2.75\scriptsize{$\pm$2.6} &1.01\scriptsize{$\pm$0.01} & \cellcolor{green!30}{3.36\scriptsize{$\pm$7.3} $\downarrow$} & \cellcolor{green!30}{0.90\scriptsize{$\pm$0.08} $\downarrow$} & \cellcolor{green!30}{69.7\scriptsize{$\pm$35.5} $\uparrow$} & \cellcolor{green!30}{45.4\scriptsize{$\pm$22.8 } $\uparrow$} \\
    & BDQ & 
        \cellcolor{green!30}{4.60{\scriptsize$\pm$0.18 $\uparrow$} } & \cellcolor{red!30}{16.67\scriptsize{$\pm$15.7}} & \cellcolor{red!30}{165.04\scriptsize{$\pm$40.99} } & \cellcolor{red!30}{5.47 \scriptsize{$\pm$2.1}}& \cellcolor{green!30}{1.00\scriptsize{$\pm$0.01}} & 3.77\scriptsize{$\pm$5.14}  & \cellcolor{red!30}{1.18\scriptsize{$\pm$0.10} } & 54.71\scriptsize{$\pm$42.75} & 28.99\scriptsize{$\pm$22.41} \\
    & LoL+ & 
        4.20{\scriptsize$\pm$0.63} & 12.52\scriptsize{$\pm$9.92} & 95.51\scriptsize{$\pm$65.0} & \cellcolor{green!30}{1.98 \scriptsize{$\pm$1.8} $\downarrow$} &1.01\scriptsize{$\pm$0.02} & 4.19\scriptsize{$\pm$7.93} &0.96\scriptsize{$\pm$0.21} & 51.19 \scriptsize{$\pm$46.19}& 30.36\scriptsize{$\pm$28.85} \\
    & Stallion & 
        \cellcolor{red!30}{3.97{\scriptsize$\pm$0.68}} & 14.26\scriptsize{$\pm$11.3} & 92.96\scriptsize{$\pm$56.24} & 2.14\scriptsize{$\pm$1.5}  &\cellcolor{red!30}{1.02\scriptsize{$\pm$0.02}} & 5.01\scriptsize{$\pm$8.15} &0.96\scriptsize{$\pm$0.18} & \cellcolor{red!30}{44.05\scriptsize{$\pm$53.66}} & \cellcolor{red!30}{25.23\scriptsize{$\pm$34.29}}\\
    & L2A & 
        4.58{\scriptsize$\pm$0.14} & 11.67\scriptsize{$\pm$8.32} & 141.85\scriptsize{$\pm$54.24}& 2.78\scriptsize{$\pm$2.7}&1.01\scriptsize{$\pm$0.02} &\cellcolor{red!30}5.50\scriptsize{$\pm$10.74} & 1.12\scriptsize{$\pm$0.14}& 67.22\scriptsize{$\pm$47.31}& 38.37\scriptsize{$\pm$26.83}\\
    \hline
    
\multirow{5}{*}{\rotatebox{90}{\textbf{Movie}}} % Merging rows 6-10
    & {\ProjectName} 
        & 3.61\scriptsize{$\pm$0.20}&4.74\scriptsize{$\pm$8.03} & \cellcolor{green!30}{74.49\scriptsize{$\pm$29.99} $\downarrow$}& 2.72\scriptsize{$\pm$2.14} &\cellcolor{green!30}{1.01\scriptsize{$\pm$0.02}} & 3.52\scriptsize{$\pm$7.68} & \cellcolor{green!30}{0.82 \scriptsize{$\pm$0.04 $\downarrow$}} & \cellcolor{green!30}{55.34\scriptsize{$\pm$43.79 $\uparrow$}} & \cellcolor{green!30}{43.67\scriptsize{$\pm$26.07 $\uparrow$}}\\
    & BDQ 
        & 4.10\scriptsize{$\pm$0.34}&\cellcolor{red!30}{40.66\scriptsize{$\pm$37.05}} & \cellcolor{red!30}{215.25\scriptsize{$\pm$84.02}} & \cellcolor{red!30}{5.90\scriptsize{$\pm$3.22}} &\cellcolor{red!30}{0.96\scriptsize{$\pm$0.01}} & \cellcolor{green!30}{3.05\scriptsize{$\pm$4.21 $\downarrow$}} & \cellcolor{red!30}{1.10\scriptsize{$\pm$0.12}} & \cellcolor{red!30}{9.25\scriptsize{$\pm$71.81}}& \cellcolor{red!30}{0.99\scriptsize{$\pm$44.39}}\\
    & LoL+ 
        & 3.50\scriptsize{$\pm$0.92}&5.18\scriptsize{$\pm$6.04} & 135.77\scriptsize{$\pm$107.00}& \cellcolor{green!30}{2.07\scriptsize{$\pm$2.15 $\downarrow$}} &1.02\scriptsize{$\pm$0.02} & 4.95\scriptsize{$\pm$8.39}& 0.94\scriptsize{$\pm$0.18}& 39.46\scriptsize{$\pm$48.54}& 23.45\scriptsize{$\pm$30.88}\\
    & Stallion 
        & \cellcolor{red!30}{3.26\scriptsize{$\pm$0.93}}&\cellcolor{green!30}{3.96\scriptsize{$\pm$5.58 $\downarrow$}} & 135.56\scriptsize{$\pm$96.59}& 2.27\scriptsize{$\pm$1.71}&1.02\scriptsize{$\pm$0.02} &5.69\scriptsize{$\pm$8.74}& 0.94\scriptsize{$\pm$0.16}& 39.23\scriptsize{$\pm$48.35} & 22.68\scriptsize{$\pm$30.44}\\
    & L2A 
        & \cellcolor{green!30}{4.10\scriptsize{$\pm$0.32} $\uparrow$}&14.20\scriptsize{$\pm$11.67} & 208.93\scriptsize{$\pm$96.99}& 4.09\scriptsize{$\pm$5.97}&1.02\scriptsize{$\pm$0.03}& \cellcolor{red!30}{9.00\scriptsize{$\pm$18.53}} & 1.07\scriptsize{$\pm$0.15}& 40.31\scriptsize{$\pm$74.49}& 23.31\scriptsize{$\pm$42.66}\\
    \hline


\multirow{5}{*}{\rotatebox{90}{\textbf{Sports}}} % Merging rows 11-15
    & {\ProjectName} 
        & 3.99\scriptsize{$\pm$0.12}&5.47\scriptsize{$\pm$7.88} &\cellcolor{green!30}{104.90\scriptsize{$\pm$13.89 $\downarrow$}} & 3.15\scriptsize{$\pm$2.58}&\cellcolor{green!30}{1.01\scriptsize{$\pm$0.02}} &4.06\scriptsize{$\pm$8.38} & \cellcolor{green!30}{0.89\scriptsize{$\pm$0.02} $\downarrow$} & \cellcolor{green!30}{ 65.19\scriptsize{$\pm$38.42} $\uparrow$} &\cellcolor{green!30}{ 41.78\scriptsize{$\pm$24.46 $\uparrow$}}\\
    & BDQ 
        & 3.77\scriptsize{$\pm$0.55}&\cellcolor{red!30}{38.27\scriptsize{$\pm$35.83}} & 136.82\scriptsize{$\pm$28.82}& \cellcolor{red!30}{18.97\scriptsize{$\pm$1.13}}&\cellcolor{red!30}{0.90\scriptsize{$\pm$0.00}} &\cellcolor{green!30}{0.51\scriptsize{$\pm$1.51 $\downarrow$}}&  0.98\scriptsize{$\pm$0.06}& \cellcolor{red!30}{4.33\scriptsize{$\pm$64.28}} & \cellcolor{red!30}{1.24\scriptsize{$\pm$39.36}}\\
    & LoL+ & 
        3.53\scriptsize{$\pm$0.86}&6.65\scriptsize{$\pm$7.64} & 128.67\scriptsize{$\pm$109.90}& \cellcolor{green!30}{2.00\scriptsize{$\pm$2.02 $\downarrow$}} &1.01\scriptsize{$\pm$0.02} & 4.14\scriptsize{$\pm$8.43}& 0.92\scriptsize{$\pm$0.18}& 48.51\scriptsize{$\pm$53.90}& 29.31\scriptsize{$\pm$35.24} \\
    & Stallion 
        & \cellcolor{red!30}{3.37\scriptsize{$\pm$0.85}} &\cellcolor{green!30}{5.39\scriptsize{$\pm$8.10 $\downarrow$}} & 130.56\scriptsize{$\pm$101.76}& 2.26\scriptsize{$\pm$1.72}& 1.02\scriptsize{$\pm$0.02}&5.06\scriptsize{$\pm$9.17}& 0.92\scriptsize{$\pm$0.16}& 49.94\scriptsize{$\pm$54.14}& 29.94\scriptsize{$\pm$35.15} \\
    & L2A 
        & \cellcolor{green!30}{4.15\scriptsize{$\pm$0.29 $\uparrow$}} &9.69\scriptsize{$\pm$10.46} & \cellcolor{red!30}{205.03\scriptsize{$\pm$103.68}} & 3.78\scriptsize{$\pm$5.21}&  1.02\scriptsize{$\pm$0.03}&\cellcolor{red!30}{ 8.12\scriptsize{$\pm$16.40} } & \cellcolor{red!30}{1.05\scriptsize{$\pm$0.16}} & 51.15\scriptsize{$\pm$68.21}  & 30.20\scriptsize{$\pm$39.63} \\
    \hline

\end{tabular}
\caption{Average Results of all metrics across testing traces for different video datasets}
\label{tab:all_results}
\end{table*}

==> mega_table_2.tex <==
\begin{table*}[ht]
\centering
% \rowcolors{3}{gray!25}{white}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \begin{tabular}{|c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|>{\columncolor{gray!25}}c|}
     
% \begin{tabular}{*11c}
\hline

% Heading row #1
% \rowcolor{white}
& \multirow{2}{*}{\textbf{ABR}} & 
\multirow{2}{*}{\textbf{Quality}} & 
\multirow{2}{*}{\textbf{Quality}} & 
\multirow{2}{*}{\textbf{Data}} & 
\multirow{2}{*}{\textbf{Latency}} & 
\multirow{2}{*}{\textbf{Speed}} & 
\multirow{2}{*}{\textbf{Freezing}} & 
\multirow{2}{*}{\textbf{Energy}} & 
\multirow{2}{*}{\textbf{QoE}} & 
\multirow{2}{*}{\textbf{Energy}} \\

% Heading row #2
% \rowcolor{white}
&  & \textbf{level} (0-5) & \textbf{Smooth} & \textbf{dl} \textit{(in Mb)} & \textit{(sec)} & & \textit{(sec)}  & \textit{(kj)} & & \textbf{Efficiency} \\
\hline
\multirow{5}{*}{\rotatebox{90}{\textbf{Animation}}}
    & {\ProjectName} & 
         4.51 & \colorbox{green!30}{10.62} & \colorbox{green!30}{87.84} & 2.75 &1.01 & \colorbox{green!30}{3.36 } & \colorbox{green!30}{0.90} & \colorbox{green!30}{69.71 } & \colorbox{green!30}{45.46 } \\
    & BDQ & 
        \colorbox{green!30}{4.60 } & \colorbox{red!30}{16.67} & \colorbox{red!30}{165.04 } & \colorbox{red!30}{5.47 }& \colorbox{green!30}{1.00} & 3.77  & \colorbox{red!30}{1.18 } & 54.71 & 28.99 \\
    & LoL+ & 
        4.20 & 12.52 & 95.51 & \colorbox{green!30}{1.98 } &1.01 & 4.19 &0.96 & 51.19 & 30.36 \\
    & Stallion & 
        \colorbox{red!30}{3.97 } & 14.26 & 92.96 & 2.14 &\colorbox{red!30}{1.02} & 5.10 &0.96 & \colorbox{red!30}{44.05} & \colorbox{red!30}{25.23}\\
    & L2A & 
        4.58 & 11.67 & 141.85& 2.78&1.01 &\colorbox{red!30}{5.50} & 1.12& 67.22& 38.37\\
    \hline
    
\multirow{5}{*}{\rotatebox{90}{\textbf{Movie}}} % Merging rows 6-10
    & {\ProjectName} 
        & 3.61&4.74 & \colorbox{green!30}{74.49}& 2.72 &\colorbox{green!30}{1.01} & 3.52 & \colorbox{green!30}{0.82 } & \colorbox{green!30}{55.34} & \colorbox{green!30}{43.67}\\
    & BDQ 
        & 4.10&\colorbox{red!30}{40.66} & \colorbox{red!30}{215.25} & \colorbox{red!30}{5.90} &\colorbox{red!30}{0.96} & \colorbox{green!30}{3.05} & \colorbox{red!30}{1.10} & \colorbox{red!30}{9.25}& \colorbox{red!30}{0.99}\\
    & LoL+ 
        & 3.50&5.18 & 135.77& \colorbox{green!30}{2.07} &1.02 & 4.95& 0.94& 39.46& 23.45\\
    & Stallion 
        & \colorbox{red!30}{3.26}&\colorbox{green!30}{3.96} & 135.56& 2.27&1.02 &5.69& 0.94& 39.2348.35 & 22.68\\
    & L2A 
        & \colorbox{green!30}{4.10}&14.20 & 209.93& 4.09&1.02& \colorbox{red!30}{9.00} & 1.07& 40.31& 23.21\\
    \hline


\multirow{5}{*}{\rotatebox{90}{\textbf{Sports}}} % Merging rows 11-15
    & {\ProjectName} 
        & 4.01&5.47 &\colorbox{green!30}{104.90} & 3.15&\colorbox{green!30}{1.01} &\colorbox{green!30}{4.06} & \colorbox{green!30}{0.89} & \colorbox{green!30}{ 65.19} &\colorbox{green!30}{ 41.78}\\
    & BDQ 
        & 3.77&\colorbox{red!30}{38.27} & 136.82& \colorbox{red!30}{8.97}&\colorbox{red!30}{0.90} &0.51&  0.98& \colorbox{red!30}{4.33} & \colorbox{red!30}{1.24}\\
    & LoL+ & 
        3.53&6.65 & 128.67& \colorbox{green!30}{2.00} &1.01 & 4.14& 0.92& 48.51& 29.31 \\
    & Stallion 
        & \colorbox{red!30}{3.37} &\colorbox{green!30}{5.39} & 130.56& 2.26& 1.02&5.06& 0.92& 49.94& 29.94 \\
    & L2A 
        & \colorbox{green!30}{4.15} &9.69 & \colorbox{red!30}{205.03} & 3.78&  1.02&\colorbox{red!30}{ 8.12 } & \colorbox{red!30}{1.05} & 51.68  & 30.20 \\
    \hline

\end{tabular}
\caption{Average Results of all metrics across testing traces for different video datasets}
\label{tab:all_results}
\end{table*}
